Cores of Games via Total Dual Integrality, with Applications to Perfect Graphs and Polymatroids

LP-duality theory has played a central role in the study of cores of games, right from the early days of this notion to the present time. The classic paper of Shapley and Shubik \cite{Shapley1971assignment} introduced the "right" way of exploiting the power of this theory, namely picking problems whose LP-relaxations support polyhedra having integral vertices. So far, the latter fact was established by showing that the constraint matrix of the underlying linear system is {\em totally unimodular}. We attempt to take this methodology to its logical next step -- {\em using total dual integrality} -- thereby addressing new classes of games which have their origins in two major theories within combinatorial optimization, namely perfect graphs and polymatroids. In the former, we address the stable set and clique games and in the latter, we address the matroid independent set game. For each of these games, we prove that the set of core imputations is precisely the set of optimal solutions to the dual LPs. Another novelty is the way the worth of the game is allocated among sub-coalitions. Previous works follow the {\em bottom-up process} of allocating to individual agents; the allocation to a sub-coalition is simply the sum of the allocations to its agents. The {\em natural process for our games is top-down}. The optimal dual allocates to "objects" in the grand coalition; a sub-coalition inherits the allocation of each object with which it has non-empty intersection.

==> Definitions.tex <==


\subsection{Definitions and Preliminary Facts}
\label{sec.matching-game}



The {\em assignment game}, $G = (U, V, E), \ w: E \rightarrow \cR_+$, has been defined in the Introduction. We start by giving definitions needed to state the Shapley-Shubik Theorem. 

\begin{definition}
	\label{sec.coalition}
		The set of all players, $U \cup V$, is called the {\em grand coalition}. A subset of the players, $(S_u \cup S_v)$, with $S_u \subseteq U$ and $S_v \subseteq V$, is called a {\em coalition} or a {\em sub-coalition}.
\end{definition}

\begin{definition}
	\label{def.worth}
	The {\em worth} of a coalition $(S_u \cup S_v)$ is defined to be the maximum profit that can be generated by teams within $(S_u \cup S_v)$ and is denoted by $p(S_u \cup S_v)$. Formally, $p(S_u \cup S_v)$ is the weight of a maximum weight matching in the graph $G$ restricted to vertices in $(S_u \cup S_v)$ only. $p(U \cup V)$ is called the {\em worth of the game}. The {\em characteristic function} of the game is defined to be $p: 2^{U \cup V} \rightarrow \cR_+$.   
\end{definition}     


\begin{definition}
	\label{def.imputation}	
	An {\em imputation}\footnote{Some authors prefer to call this a pre-imputation, while using the term imputation when individual rationality is also satisfied.} gives a way of dividing the worth of the game, $p(U \cup V)$, among the agents. It consists of two functions $u: {U} \rightarrow \cR_+$ and $v: {V} \rightarrow \cR_+$ such that $\sum_{i \in U} {u(i)} + \sum_{j \in V} {v(j)} = p(U \cup V)$. 
\end{definition}
	
\begin{definition}
	\label{def.core}
	An imputation $(u, v)$ is said to be in the {\em core of the assignment game} if for any coalition $(S_u \cup S_v)$, the total worth allocated to agents in the coalition is at least as large as the worth that they can generate by themselves, i.e., $\sum_{i \in S_u} {u(i)} +  \sum_{j \in S_v} {v(j)} \geq p(S)$.
\end{definition}
 
We next describe the characterization of the core of the assignment game given by Shapley and Shubik \cite{Shapley1971assignment}\footnote{Shapley and Shubik had described this game in the context of the housing market in which agents are of two types, buyers and sellers. They had shown that each imputation in the core of this game gives rise to unique prices for all the houses. In this paper we will present the assignment game in a variant of the tennis setting given in the Introduction; this will obviate the need to define ``prices'', hence leading to simplicity.}. 

As stated in Definition \ref{def.worth}, the worth of the game, $G = (U, V, E), \ w: E \rightarrow \cR_+$, is the weight of a maximum weight matching in $G$. Linear program (\ref{eq.core-primal-bipartite}) gives the LP-relaxation of the problem of finding such a matching. In this program, variable $x_{ij}$ indicates the extent to which edge $(i, j)$ is picked in the solution. Matching theory tells us that this LP always has an integral optimal solution \cite{LP.book}; the latter is a maximum weight matching in $G$.

	\begin{maxi}
		{} {\sum_{(i, j) \in E}  {w_{ij} x_{ij}}}
			{\label{eq.core-primal-bipartite}}
		{}
		\addConstraint{\sum_{(i, j) \in E} {x_{ij}}}{\leq 1 \quad}{\forall i \in U}
		\addConstraint{\sum_{(i, j) \in E} {x_{ij}}}{\leq 1 }{\forall j \in V}
		\addConstraint{x_{ij}}{\geq 0}{\forall (i, j) \in E}
	\end{maxi}

Taking $u_i$ and $v_j$ to be the dual variables for the first and second constraints of (\ref{eq.core-primal-bipartite}), we obtain the dual LP: 

 	\begin{mini}
		{} {\sum_{i \in U}  {u_{i}} + \sum_{j \in V} {v_j}} 
			{\label{eq.core-dual-bipartite}}
		{}
		\addConstraint{ u_i + v_j}{ \geq w_{ij} \quad }{\forall (i, j) \in E}
		\addConstraint{u_{i}}{\geq 0}{\forall i \in U}
		\addConstraint{v_{j}}{\geq 0}{\forall j \in V}
	\end{mini}


\begin{theorem}
	\label{thm.SS}
	(Shapley and Shubik \cite{Shapley1971assignment})
	The imputation $(u, v)$ is in the core of the assignment game if and only if it is an optimal solution to the dual LP, (\ref{eq.core-dual-bipartite}). 
\end{theorem}
	

By Theorem \ref{thm.SS}, the core of the assignment game is a convex polyhedron. Shapley and Shubik shed further light on the structure of the core by showing that it has two special imputations which are furtherest apart and so can be thought of as antipodal imputations. In the tennis club setup, one of these imputations maximizes the earnings of women players and the other maximizes the earnings of men players. These are illustrated in Examples \ref{ex.3} and \ref{ex.4}. 

Finally, we state a fundamental fact about LP (\ref{eq.core-primal-bipartite}); its corollary will be used in a crucial way in Theorems \ref{thm.vertices} and \ref{thm.edges}.

\begin{theorem}
	\label{thm.Birkhoff}
	(Birkhoff \cite{Birkhoff1946three})	The vertices of the polytope defined by the constraints of LP (\ref{eq.core-primal-bipartite}) are $0/1$ vectors, i.e., they are matchings in $G$.
\end{theorem}


\begin{corollary}
	\label{cor.Birkhoff}
	Any fractional matching in a bipartite graph is a convex combination of integral matchings. 
\end{corollary}







 
